Unfolding-based Partial Order Reduction

Partial order reduction (POR) and net unfoldings are two alternative methods to tackle state-space explosion caused by concurrency. In this paper, we propose the combination of both approaches in an effort to combine their strengths. We first define, for an abstract execution model, unfolding semantics parameterized over an arbitrary independence relation. Based on it, our main contribution is a novel stateless POR algorithm that explores at most one execution per Mazurkiewicz trace, and in general, can explore exponentially fewer, thus achieving a form of super-optimality. Furthermore, our unfolding-based POR copes with non-terminating executions and incorporates state-caching. Over benchmarks with busy-waits, among others, our experiments show a dramatic reduction in the number of executions when compared to a state-of-the-art DPOR.

==> model.tex <==
\section{Model of Computation}
\label{s:model}

We consider an abstract model of concurrent computation,
general enough to capture any reasonable means of process interaction,
such as shared memory or message passing.
Our model represents a finite number of concurrent, finite-state processes
that communicate by means of some finite shared state.

Formally, a \emph{system} is a tuple
$M \eqdef \tup{\Sigma, T, \tilde s}$ formed by
a set~$\Sigma$ of \emph{global states},
a set~$T$ of \emph{transitions}, and some
\emph{initial global state} $\tilde s \in \Sigma$.
Each transition $t \colon \Sigma \to \Sigma$ in~$T$ is
a \emph{partial} function accounting for how the occurrence of~$t$
transforms the state of~$M$.

%For a system with~$n$ processes,
%traditionally~$T$ is presented as being the disjoint union
%$T_1 \uplus \ldots \uplus T_n$ of $n$ sets~$T_i$, each one containing the
%transitions of process~$i$.
%This distinction is irrelevant for the developpments in this paper.

%Transitions may belong to more than one process, \ie,
%$T_i \cap T_j$ is not necessarily empty for $i \ne j$.
%We denote by $\proc t$ the set of process identifiers
%to which it belongs, formally
%$\proc t \eqdef
%\set{i \in \set{1, \ldots, n} \colon t \in T_i}$.

A transition $t \in T$ is \emph{enabled} at a state~$s$ if~$t(s)$ is defined.
Such~$t$ can \emph{fire} at~$s$, producing a new state $s' \eqdef t (s)$.
We let $\enabl s$ denote the set of transitions enabled at~$s$.
The \emph{interleaving semantics} of $M$ is the
directed, edge-labelled graph
$\intsem M \eqdef \tup{\Sigma, {\to}, \tilde s}$ where
$\Sigma$ are the global states,
$\tilde s$ is the initial state and
${\to} \subseteq \Sigma \times T \times \Sigma$
contains a triple $\tup{s, t, s'}$, denoted by $s \fire t s'$, iff~$t$ is
enabled at~$s$ and~$s' = t(s)$.
Given
two states $s, s' \in \Sigma$, and
$\sigma \eqdef t_1.t_2 \ldots t_n \in T^*$
($t_1$~concatenated with~$t_2$, \ldots until~$t_n$),
we denote by $s \fire{\sigma} s'$
the fact that there exist states $s_1, \ldots, s_{n-1} \in \Sigma$ such that
$s \fire{t_1} s_1$, \ldots, $s_{n-1} \fire{t_n} s'$.

A \emph{run} (or \emph{interleaving}, or \emph{execution})
of $M$ is any sequence $\sigma \in T^*$ such that
$\tilde s \fire \sigma s$ for some $s \in \Sigma$.
We denote by~$\state \sigma$ the state~$s$ that $\sigma$ reaches,
and by~$\runs M$ the set of runs of~$M$, also referred to as the
\emph{interleaving space}.
A state~$s \in \Sigma$ is \emph{reachable}
if $s = \state \sigma$ for some $\sigma \in \runs M$;
it is a \emph{deadlock} if $\enabl s = \emptyset$, and in that
case~$\sigma$ is called \emph{maximal}, or \emph{deadlocking}.
We let $\reach M$ denote the set of reachable states in~$M$.

For the rest of the paper,
we fix a system~$M \eqdef \tup{\Sigma, T, \tilde s}$ and assume that
(i) $\reach M$ is finite and that
(ii) each transition in~$T$ is a function decidable in polynomial time.

%FIXME
% - linearizations of a partial order
% - labelled partial orders,


